The Effect of Human v/s Synthetic Test Data and Round-tripping on Assessment of Sentiment Analysis Systems for Bias

Sentiment Analysis Systems (SASs) are data-driven Artificial Intelligence (AI) systems that output polarity and emotional intensity when given a piece of text as input. Like other AIs, SASs are also known to have unstable behavior when subjected to changes in data which can make it problematic to trust out of concerns like bias when AI works with humans and data has protected attributes like gender, race, and age. Recently, an approach was introduced to assess SASs in a blackbox setting without training data or code, and rating them for bias using synthetic English data. We augment it by introducing two human-generated chatbot datasets and also consider a round-trip setting of translating the data from one language to the same through an intermediate language. We find that these settings show SASs performance in a more realistic light. Specifically, we find that rating SASs on the chatbot data showed more bias compared to the synthetic data, and round-tripping using Spanish and Danish as intermediate languages reduces the bias (up to 68% reduction) in human-generated data while, in synthetic data, it takes a surprising turn by increasing the bias! Our findings will help researchers and practitioners refine their SAS testing strategies and foster trust as SASs are considered part of more mission-critical applications for global use.

==> sections/discussion.tex <==
\section{Discussion}
\kl{Prof. Biplav, can you fill this?}

==> sections/ethics.tex <==
\section{Limitations}
Here are a few limitations of our work: 
\begin{itemize}
    \item Currently, the rating method gives the intensity of the bias for a protected variable but does not give information on how biased a system is towards a particular values of the protected attribute. For example, would the given raw score indicate bias towards a specific value (e.g., male) of a protected attribute like gender? We treated it outside of the current scope and leave it as future work. 
    
    \item We used Google translate for round-trip translating. In future, more translators could be used. We used round-trip translation in the paper for two intermediate languages - Spanish and Danish. One could extend with other hundreds of languages supported by a modern learning-based translator like Google Translate. Currently, all results are computed in the context of SASs in English. If training data or SASs trained on data in other languages were  available, this method can be used to rate SASs using other language test datasets.
    
    \item We evaluated SASs on human-generated chatbot data collected from two different domains (playing games and university information). However, there can be domains where sentiment may be more critical, like healthcare and finance. So, if human-generated datasets in  areas like these are made available, the rating method can be used to evaluate SASs on that data and can help more socially critical applications. 
    
    \item We considered representative systems from each category (learning-based, lexicon-based, large language models (LLM) based,  custom). However, more sentiment system types and implementations within them can be considered. For example, in LLMs, where there are many new models released recently and especially with support for multiple modes like text, audio and video. %LLMs can be evaluated for bias on sentiment analysis task as a part of future work.
\end{itemize}

\section{Ethics Statement}
In our work, we assess Sentiment Analysis Systems (SASs) for bias using human-generated and round-trip translated data. In \cite{sas-rating}, the authors stated that a system is biased when any of the protected attributes are affecting the system outcome. We agree with that and adhere to the same definition throughout the paper. We discuss the motivation and significance of the work in Sections \ref{sec:introduction} and \ref{sec:background}.  We define the problem in a concrete and formal manner in Section \ref{sec:problem}. We performed many experiments (Section \ref{expts}) with clearly defined goals and setup. The final interpretations and conclusion (Section \ref{sec:interpret}) drawn from each experiment would help developers and practitioners in refining the AI testing strategies for building more trustworthy applications. 

The human-generated datasets we used were collected from human studies in an ethical manner with consent. Participants  names were not collected and participant confidentiality was maintained. IRB numbers are provided in the supplementary material (Section C). Section F has the annotation protocols (complete instructions that were provided to the annotators). We assure that our research was conducted in accordance with the highest ethical standards.
